Capacity Region of Layered Erasure One-sided Interference Channels without CSIT

This paper studies a layered erasure interference channel model, which is a simplification of the Gaussian interference channel with fading using the deterministic model approach. In particular, the capacity region of the layered erasure one-sided interference channel is completely determined, assuming that the channel state information (CSI) is known to the receivers, but there is no CSI at transmitters (CSIT). The result holds for arbitrary fading statistics. Previous results of Aggarwal, Sankar, Calderbank and Poor on the capacity region or sum capacity under several interference configurations are shown to be special cases of the capacity region shown in this paper.

==> figs/figCap.tex <==
\begin{tikzpicture}[scale=.6]
        \coordinate (origin) at (0, 0);
      \draw[->, ultra thick] (0,0) -- (6,0) node[below] {$R_1$};
        \draw[->, ultra thick] (0,0) -- (0, 8.5) node[left] {$R_2$};
        \coordinate (C1) at (4,0);
        \coordinate (C11) at (4,10);
        \coordinate (C2) at (0,6);
        \coordinate (C22) at (10,6);
        % points on lines
        \coordinate (L1x) at (4.5,0);
        \coordinate (L1y) at (0,13.5);
        \coordinate (L2x) at (5,0);
        \coordinate (L2y) at (0,10);
        \coordinate (L3x) at (5.8,0);
        \coordinate (L3y) at (0,8.7);
        \coordinate (L4x) at (8,0);
        \coordinate (L4y) at (0,8);
        % cross points
        \coordinate (L0) at (intersection of C1--C11 and L1x--L1y);
        \coordinate (L1) at (intersection of L1x--L1y and L2x--L2y);
        \coordinate (L2) at (intersection of L2x--L2y and L3x--L3y);
        \coordinate (L3) at (intersection of L3x--L3y and L4x--L4y);
        
        %draw segments
        \draw[very thick] (C1) node [below]{\small $\MEXP \rN_{1}$}--(L0);
        \draw[very thick] (L0) --node[right]{$1\wedge \omega_1$} (L1);
        \draw[very thick] (L1)node[right]{$L_1$} --node[right]{$1 \wedge \omega_2$} (L2)node[right]{$L_2$};
        \coordinate (up) at (intersection of C2--C22 and L2--L3);
        \draw[very thick] (C2) node[left]{\small$\MEXP \rN_{2}$}--(up);
        \draw[very thick] (up)--(L2);
        \draw[very thick] (L3)node[right]{$L_3$} --node[right]{$1\wedge \omega_4$} (L4y);
        \draw[very thick] (L3) -- node[right]{$1\wedge \omega_3$}(L2);
        \fill[black] (C1) circle (1mm);
        \fill[black] (C2) circle (1mm);
        \node[rectangle, inner sep=1mm,draw=blue, fill=blue] at (L0) {};
        \node[rectangle, inner sep=1mm,draw=blue, fill=blue] at (up) {};
       \node[star, inner sep=.6mm,draw=red, fill=red] at (L1) {};
        \node[star, inner sep=.6mm,draw=red, fill=red] at (L2) {};
        \node[star, inner sep=.6mm,draw=red, fill=red] at (L3) {};
        \draw[dashed] (L0) --( L0 -| C2) node[left]{\small $\MEXP \left[\rN_{0}
            - \rN_{1} \right]^+$};
\end{tikzpicture}




%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../Z_RCSI"
%%% End: 


==> figs/figGauOuter.tex <==
\begin{tikzpicture}
        \coordinate (origin) at (0, 0);
      \draw[->, ultra thick] (0,0) -- (8.5,0) node[below] {$R_1$};
        \draw[->, ultra thick] (0,0) -- (0, 8.5) node[left] {$R_2$};
        \coordinate (C1) at (5,0);
        \coordinate (C11) at (5,1.5);
        \coordinate (C2) at (0,6.5);
        \coordinate (C22) at (10,6.5);
        \coordinate (cor) at (1,6);
        \draw  (C1) -- (C11);
        \draw (C11) -- (cor);
\end{tikzpicture}


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../Z_RCSI"
%%% End: 


==> figs/figQ1Ach1.tex <==
    \begin{tikzpicture}[scale=.8]
        \draw [<->,ultra thick] (0,5) node (yaxis) [above] {$R_2$}
        |- (5,0) node (xaxis) [right] {$R_1$};
        \coordinate (origin) at (0,0);
        \coordinate  (r_2) at (0,3);
        \coordinate  (r_22) at (10,3);
        \coordinate  (r_1) at (3,0);
        \coordinate  (r_11) at (3,10);
        \coordinate  (r_3) at (0,1);
        \coordinate  (r_33) at (10,1);
        \coordinate  (a_2) at (0,4.5);
        \coordinate  (a_1) at (4.5,0);
        \coordinate (a) at (intersection of r_2--r_22 and a_1--a_2);
        \draw[dashed] (r_2) node[left]{$\Ces_{0}$}-- (a);
        \coordinate (c) at (intersection of r_3--r_33 and r_1--r_11);
        \draw[very thick] (r_3) node[left]{$\Ces_{2}$}--(c);
        \draw[dashed] (a_1) -- (a_2);
        % \draw[dashed] (a) -- (a_2);
        \coordinate (b) at (intersection of a_1--a_2 and r_1--r_11); 
        %\draw (a) -- (b);
        \draw[dashed] (b)--(c);
        \draw[very thick] (c)--(r_1) node[below]{\small$\Ces_{1}$};
        % \draw[dashed] (b)--(a_1);
        \draw[dashed] (b)--(0,1.5) node[left]{\small $\Ces_{0}\epsilon_{1}$};
        \draw[dashed] (a)--(1.5,0) node[below]{\small $\Ces_{1}\epsilon_{0}$};
        \fill[black] (r_2) circle (1mm);
        \fill[black] (r_1) circle (1mm);
        \draw [->] (3.3,3.3) node[above] {\small$\tiny R_1 + R_2 = \Ces_{0} +
          \Ces_{1} - \Ces_{0} \Ces_{1}$}--(2.4,2.4);
        \fill[nearly transparent, green!70!white] (r_2)--(a)--(b)--(r_1)--(origin)--cycle;
      \end{tikzpicture}




%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../Z_RCSI"
%%% End: 


==> figs/figQ1Ach2.tex <==
    \begin{tikzpicture}[scale=.8]
        \draw [<->,ultra thick] (0,5) node (yaxis) [above] {$R_2$}
        |- (5,0) node (xaxis) [right] {$R_1$};
        \coordinate (origin) at (0,0);
        \coordinate  (r_2) at (0,3);
        \coordinate  (r_22) at (10,3);
        \coordinate  (r_1) at (3,0);
        \coordinate  (r_11) at (3,10);
        \coordinate  (r_3) at (0,2.5);
        \coordinate  (r_33) at (10,2.5);
        \coordinate  (a_2) at (0,4.5);
        \coordinate  (a_1) at (4.5,0);
        \coordinate (a) at (intersection of r_2--r_22 and a_1--a_2);
        \draw[dashed] (r_2) node[left]{$\Ces_{0}$}-- (a);
        \draw[dashed] (a_1) -- (a_2);
        \coordinate (b) at (intersection of a_1--a_2 and r_1--r_11);
        \coordinate (e) at (1.5,0);
        \coordinate (d) at (intersection of a--e and origin--a_1);
        \draw[very thick] (b)--(r_1) node[below]{\small $\Ces_{1}$};
        \draw[dashed] (a)--(d)node[below]{\small$\Ces_{1}\epsilon_0$};
        \coordinate (c) at (intersection of r_3--r_33 and a_1--a_2);
        \draw[very thick] (r_3) node[left]{$\Ces_{2}$}--(c);
        \draw[very thick] (c)--(b);
        \fill[black] (r_2) circle (1mm);
        \fill[black] (r_1) circle (1mm);
        %\fill[red] (c) circle (1mm);
        \node[star, inner sep=.6mm,draw=red, fill=red] at (c) {};
        \node[rectangle, inner sep=1mm,draw=blue, fill=blue] at (b) {};
        \draw [->] (3.3,3.3) node[above] {\small$\tiny R_1 + R_2 = \Ces_{0} +
          \Ces_{1} - \Ces_{0} \Ces_{1}$}--(2.4,2.4);
        \coordinate (f) at (0,1.5);
        \draw[dashed] (b)--(0,1.5) node[left]{\small $\Ces_{0}\epsilon_1$};
        \fill[nearly transparent, green!70!white] (r_2)--(a)--(b)--(r_1)--(origin)--cycle;
      \end{tikzpicture}



%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "Z_RCSI"
%%% End: 


==> figs/figQ1Ach3.tex <==
    \begin{tikzpicture}[scale=.8]
        \draw [<->,ultra thick] (0,5) node (yaxis) [above] {$R_2$}
        |- (5,0) node (xaxis) [right] {$R_1$};
        \coordinate (origin) at (0,0);
        \coordinate  (r_2) at (0,3);
        \coordinate  (r_22) at (10,3);
        \coordinate  (r_1) at (3,0);
        \coordinate  (r_11) at (3,10);
        \coordinate  (r_3) at (0,3.5);
        \coordinate  (r_33) at (10,3.5);
        \coordinate  (a_2) at (0,4.5);
        \coordinate  (a_1) at (4.5,0);
        \coordinate (a) at (intersection of r_2--r_22 and a_1--a_2);
        \draw[dashed] (r_2) node[left]{$\Ces_{0}$}-- (a);
        \draw[dashed] (a_1) -- (a_2);
        \coordinate (b) at (intersection of a_1--a_2 and r_1--r_11);
        \coordinate (e) at (1.5,0);
        \coordinate (d) at (intersection of a--e and origin--a_1);
        \draw[very thick] (b)--(r_1) node[below]{\small $\Ces_{1}$};
        \draw[dashed] (a)--(d)node[below]{\small$\Ces_{1}\epsilon_0$};
        \coordinate (c) at (intersection of r_3--r_33 and a--e);
        \draw[very thick] (r_3) node[left]{$\Ces_{2}$}--(c);
        \draw[very thick] (c)--(b);
        \draw[dashed] (a)--(c);
        \fill[black] (r_2) circle (1mm);
        \fill[black] (r_1) circle (1mm);
        \node[star, inner sep=.6mm,draw=red, fill=red] at (c) {};
        \node[rectangle, inner sep=1mm,draw=blue, fill=blue] at (b) {};
        \draw [->] (3.5,4) node[above] {\small$\tiny R_1 + R_2 = \Ces_{0} +
          \Ces_{1} - \Ces_{0} \Ces_{1}$}--(1.8,2.8);
      \coordinate (f) at (0,1.5);
        \draw[dashed] (b)--(0,1.5) node[left]{\small $\Ces_{0}\epsilon_{1}$};
        \fill[nearly transparent, green!70!white] (r_2)--(a)--(b)--(r_1)--(origin)--cycle;
      \end{tikzpicture}


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "Z_RCSI"
%%% End: 


==> zycommandset.tex <==
\newtheorem{theorem}{Theorem}
\newtheorem{prop}{Proposition}
\newtheorem{lemma}{Lemma}
\newtheorem{coro}[theorem]{Corollary}
\newtheorem{defi}{Definition}
\newtheorem{algo}{Algorithm}
\newtheorem{remark}{Remark}
\newtheorem{example}{Example}
\newtheorem{conj}{Conjecture}

\newcommand{\mbA}{\mathbf{A}}
\newcommand{\mbB}{\mathbf{B}}
\newcommand{\mbC}{\mathbf{C}}
\newcommand{\mbD}{\mathbf{D}}
\newcommand{\mbE}{\mathbf{E}}
\newcommand{\mbF}{\mathbf{F}}
\newcommand{\mbG}{\mathbf{G}}
\newcommand{\mbH}{\mathbf{H}}
\newcommand{\mbI}{\mathbf{I}}
\newcommand{\mbJ}{\mathbf{J}}
\newcommand{\mbK}{\mathbf{K}}
\newcommand{\mbL}{\mathbf{L}}
\newcommand{\mbM}{\mathbf{M}}
\newcommand{\mbN}{\mathbf{N}}
\newcommand{\mbO}{\mathbf{O}}
\newcommand{\mbP}{\mathbf{P}}
\newcommand{\mbQ}{\mathbf{Q}}
\newcommand{\mbR}{\mathbf{R}}
\newcommand{\mbS}{\mathbf{S}}
\newcommand{\mbT}{\mathbf{T}}
\newcommand{\mbU}{\mathbf{U}}
\newcommand{\mbV}{\mathbf{V}}
\newcommand{\mbW}{\mathbf{W}}
\newcommand{\mbX}{\mathbf{X}}
\newcommand{\mbY}{\mathbf{Y}}
\newcommand{\mbZ}{\mathbf{Z}}

\newcommand{\mba}{\mathbf{a}}
\newcommand{\mbb}{\mathbf{b}}
\newcommand{\mbc}{\mathbf{c}}
\newcommand{\mbd}{\mathbf{d}}
\newcommand{\mbe}{\mathbf{e}}
\newcommand{\mbf}{\mathbf{f}}
\newcommand{\mbg}{\mathbf{g}}
\newcommand{\mbh}{\mathbf{h}}
\newcommand{\mbi}{\mathbf{i}}
\newcommand{\mbj}{\mathbf{j}}
\newcommand{\mbk}{\mathbf{k}}
\newcommand{\mbl}{\mathbf{l}}
\newcommand{\mbm}{\mathbf{m}}
\newcommand{\mbn}{\mathbf{n}}
\newcommand{\mbo}{\mathbf{o}}
\newcommand{\mbp}{\mathbf{p}}
\newcommand{\mbq}{\mathbf{q}}
\newcommand{\mbr}{\mathbf{r}}
\newcommand{\mbs}{\mathbf{s}}
\newcommand{\mbt}{\mathbf{t}}
\newcommand{\mbu}{\mathbf{u}}
\newcommand{\mbv}{\mathbf{v}}
\newcommand{\mbw}{\mathbf{w}}
\newcommand{\mbx}{\mathbf{x}}
\newcommand{\mby}{\mathbf{y}}
\newcommand{\mbz}{\mathbf{z}}

\newcommand{\ud}{\mathrm{d}}
\newcommand{\uT}{\mathrm{T}}
\newcommand{\uH}{\mathrm{H}}


\newcommand{\fixme}[1]{{\color{red} #1}}
\newcommand{\modify}[1]{{\color{blue} #1}}
\newcommand{\comment}[1]{{\color{green} #1}}

==> zymacroset.tex <==
\usepackage{ifthen}

\newtheorem{theorem}{Theorem}
\newtheorem{prop}{Proposition}
\newtheorem{lemma}{Lemma}
\newtheorem{coro}[theorem]{Corollary}
\newtheorem{defn}{Definition}
\newtheorem{algo}{Algorithm}
\newtheorem{remark}{Remark}
\newtheorem{example}{Example}
\newtheorem{conj}{Conjecture}
\newtheorem{claim}{Claim}

\ifthenelse{\equal{\dongningstyle}{true}}{
        \newcommand{\RVEC}[1]{\boldsymbol{\uppercase{#1}}}
        \newcommand{\RMAT}[1]{\underline{\boldsymbol{\uppercase{#1}}}}
        \newcommand{\RSCA}[1]{\uppercase{#1}}
        \newcommand{\VEC}[1]{\boldsymbol{\lowercase{#1}}}
        \newcommand{\MAT}[1]{\boldsymbol{\underline{\lowercase{#1}}}}
}{
        \newcommand{\RVEC}[1]{\boldsymbol{#1}}
        \newcommand{\RMAT}[1]{\boldsymbol{\mathrm{\uppercase{#1}}}}
        \newcommand{\RSCA}[1]{\boldsymbol{#1}}
        \newcommand{\VEC}[1]{#1}
        \newcommand{\MAT}[1]{\mathrm{\uppercase{#1}}}
}




\newcommand{\snr}{\mathsf{snr}}
\newcommand{\mmse}[1]{\mathsf{mmse}\left[ #1 \right]}
\newcommand{\inr}{\mathsf{INR}}
\newcommand{\MEXP}{\mathbb{E}}
\newcommand{\Prob}[1]{\mathsf{P}\left( #1 \right)}
\newcommand{\Probb}{\mathsf{P}}
\newcommand{\LOG}[1]{\log \left( #1 \right)}
\newcommand{\HAT}[1]{\widehat{#1}}
\newcommand{\TIT}[1]{\widetilde{#1}}
\newcommand{\FLR}[1]{\lfloor #1 \rfloor}
\allowdisplaybreaks

\newcommand{\uT}{\mathsf{T}}
\newcommand{\ud}{\mathsf{d}}
\newcommand{\trace}{\mathsf{tr}}


\newcommand{\fixme}[1]{{\color{Orangered} #1}}
\newcommand{\modify}[1]{{\color{Navyblue} #1}}

